Probabilistic Decoupling of Labels in Classification

We investigate probabilistic decoupling of labels supplied for training, from the underlying classes for prediction. Decoupling enables an inference scheme general enough to implement many classification problems, including supervised, semi-supervised, positive-unlabelled, noisy-label and suggests a general solution to the multi-positive-unlabelled learning problem. We test the method on the Fashion MNIST and 20 News Groups datasets for performance benchmarks, where we simulate noise, partial labelling etc.

==> tex/iterative_inference.tex <==



Say we have approximated the selection label matrix $\widehat{\bS}$, and inferred a transition matrix $\widehat{\bT}$ and some class distributions $\widehat{\bY}$ as described in the previous section. Ideally these class distributions will be close to the true class distributions for the samples, but due to limited data this may not be the case. Noisy labels can make classes have mass in regions of the input space where they shouldn't, and some regions may only have unlabelled samples (or none). For helping with these problems it will be useful to iteratively update our beliefs about the class and selection probabilities, and our training samples. This will allow us to propagate label and class probabilities onto unlabelled samples, and to correct samples that were mislabelled {\color{red} Cite Label Propagation paper}. 

Using $\widehat{\bY}$ and $\widehat{\bT}$, we could create a new $\bS$, which we could train a new $g(\bx) \approx p(\bs \given \bx)$ on. We could then iteratively apply this method in hope of convergence to the true distributions of $\bS$, $\bT$ and $\bY$. This idea is very circular and does not take advantage of the original selection labels after the first iteration. Furthermore the selection labels are (due to possible noise-elements in the transition) "watered-down", mixed versions of the true labels we search for. The whole system will therefore converge to a mixed-label solution. 

\subsection{Iterative Algorithm}

We will therefore attempt to get from selection domain to class domain from the first iteration, and then handle task \ref{task:iter_update_Y_T_from_SD}, where we iteratively update our beliefs about the class domain while conditioning on the original selections. This algorithm is outlined in Algorithm \ref{alg:iterative_inference}. Lines \ref{algl:train_g(x)}-\ref{algl:first_inference} performs the inference of both $\bT$ and $\bY$ using the method of section \ref{sec:inference_Y_T}. Line \ref{algl:est_W0} estimates the class probabilities of the samples of the dataset conditioned on the selections. These class probabilities are iteratively updated and used for training a classifier to estimate the class densities over the input space, in the loop starting at line \ref{algl:iter_inference_start}. Line \ref{algl:est_Wi} ensures our beliefs on the training samples are conditioned on their selections. 


\begin{algorithm}
	\begin{spacing}{1.4}
		\caption{Iterative Inference Method} \label{alg:iterative_inference}
		\begin{algorithmic}[1]
			\Statex Dataset: $\bX, \bS_{\mathcal{D}}$
			\State Train $g(\bx) \approx p(\bs \given \bx)$ on $\bS_{\mathcal{D}}$  \label{algl:train_g(x)}
			\State Use $g(\bx)$ to make $\widehat{\bS} \approx p(\bS \given \bX)$
			\State Use $\widehat{\bS}$ to infer $\widehat{\bT}_0$ and $\widehat{\bY}_0 \approx p(\by \given \bx)$ \hfill task \ref{task:infer_Y_T_from_S} \label{algl:first_inference}
			\State Use $\widehat{\bY}_0$, $\widehat{\bT}_0$, $\bS_{\mathcal{D}}$ to estimate $\widehat{\bW}_0 \approx p(y \given \bx, s)$ \hfill task \ref{task:est_W_from_Y_T_SD} \label{algl:est_W0}
			\Statex \vspace{-5mm}
			%
			\vspace{2mm}\For{i $\in [0 .. n]$ } \hfill task \ref{task:iter_update_Y_T_from_SD}  \label{algl:iter_inference_start}
			\State Train $f(\bx) \approx p(\by \given \bx)$ on $\widehat{\bW}_i$
			\State Evaluate $f(\bx)$ to create $\widehat{\bY}_{i + 1}$
			\State Use $\widehat{\bY}_{i + 1}$, $\bS_{\mathcal{D}}$ to estimate  $\widehat{\bT}_{i+1}$ \hfill task \ref{task:est_T_from_Y_SD}
			\State Use $\widehat{\bY}_{i + 1}$, $\widehat{\bT}_{i+1}$, $\bS_{\mathcal{D}}$ to estimate $\widehat{\bW}_{i+1}$ \hfill task \ref{task:est_W_from_Y_T_SD} \label{algl:est_Wi}
			\EndFor
		\end{algorithmic}
	\end{spacing}
\end{algorithm}


\subsection{Thoughts on Inference Using Lemma}

\note{Try this experiment with extremely small kernels.}

In the first inference problem we train $g(\bx) \approx p(\bs \given \bx)$ to make $\widehat{\bS}$, and then use $\widehat{\bS}$ to infer $\widehat{\bT}$ and $\widehat{\bY} \approx p(\by \given \bx)$. 
Say we used an extremely flexible model for $g(\bx)$ (for example a kernel density estimator with an extremely small kernel). Using this model will provide $\widehat{\bS} \approx \bS_{\mathcal{D}}$, which results in the following
\begin{enumerate}[itemsep=0pt, topsep=0pt]
	\item The problem degrades to simply estimating a class distribution for each selection, which is solely based on the prior of $\bT$, as the input space is never used. $\bS_{\mathcal{D}}$ only has as many unique rows as there are classes (is very singular), and so there will be one solution for each of these rows. 
	\item It will not make any sense to apply the model to new samples, as the model will be evaluated in regions of the classifier with no training information and $\bT$ is only optimized for one-hot selection distributions. 
\end{enumerate}
We thus rely on the inflexibility (the regularization) of the model to provide non-singular distributions for $\widehat{\bS}$ and to provide predictions for samples that are more distant from the training data. 

Another thing to note is that if an algorithm is trained on a dataset and then evaluated on the same dataset, then these probabilities will be biased towards the selections of the training set. For the optimal performance of this inference, one might therefore have to apply a cross-prediction or leave-one-out-prediction scheme (which may be costly). The same can be said about the classifier $f(\bx)$ used for modelling $p(y \given \bx)$ within the loop of the iterative method. \\
If we want the method to work without cross-prediction or leave-one-out-prediction, then we again rely on the inflexibility and regularization of the model, to force the selection and class distributions to mix and become non-singular. 

Finally in order for labels to propagate to unlabelled data, we again need inflexibility of the model to force labels from nearby labelled data onto unlabelled data. 

If ones only goal is to best estimate $\bW$ from $\bS_{\mathcal{D}}$, and not do future prediction, then the models for $g(\bx)$ and $f(\bx)$ are still needed, and will be used to ensure rigidness of the class and selection distributions in the input space. 

Another aspect of using this algorithm is the choice of $g(\bx)$ and $f(\bx)$. They estimate different probabilities but operate on the same input space. If there is a large difference in the number of selection labels and classes, we may need a different classification model for $g(\bx)$ and $f(\bx)$, although in most cases we believe that the same model can simply be applies. In situations where there is a one-to-one correspondence between selection labels and classes (which is really most classical classification tasks) the two functions end up learning the same thing, and there is no need to consider their differences. 

